CEPA: Consensus Embedded Perturbation for Agnostic Detection and Inversion of Backdoors

A variety of defenses have been proposed against Trojans planted in (backdoor attacks on) deep neural network (DNN) classifiers. Backdoor-agnostic methods seek to reliably detect and/or to mitigate backdoors irrespective of the incorporation mechanism used by the attacker, while inversion methods explicitly assume one. In this paper, we describe a new detector that: relies on embedded feature representations to estimate (invert) the backdoor and to identify its target class; can operate without access to the training dataset; and is highly effective for various incorporation mechanisms (i.e., is backdoor agnostic). Our detection approach is evaluated -- and found to be favorable - in comparison with an array of published defenses for a variety of different attacks on the CIFAR-10 and CIFAR-100 image-classification domains.

==> Section/CEPA-fig1-4.tex <==
Acting on layer 5 of the ResNet18 model,
Figures \ref{fig:layer5-consensus} and \ref{fig:layer5-norm} 
respectively show the performance of our defense in terms of 
the consensus measure consisting of the estimated standard deviation 
divided by the L2 norm of $\mu$, $\sigma/\|\mu\|$, and in terms of $\|\mu\|$,
on four typical poisoned models and on an typical unattacked (clean) model.
Figures \ref{fig:layer13-consensus} and \ref{fig:layer13-norm} show the
same measures for layer 13, where the ground truth target class of the attack is in red.
From the bar charts (one bar for each {\em putative} target class), one can see that, for both layers 5 and 13, CEPA strongly indicates the true target class (9) on poisoned models, i.e., the quantities for the true target class are clear outliers with respect those for the non-target classes (0-8), but does not indicate any significant outliers in the case of a clean model (i.e., there are no false positive class detections). 
The exception is the global chessboard backdoor, which is only clearly detected using layer 5.
%We again note that our method can be applied to a {\em plurality} of layers (embedded feature representations) of the model to detect backdoor poisoning.



\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/BadNet_L5_consensus.png}
         \caption{BadNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/WaNet_L5_consensus.png}
         \caption{WaNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Chess_L5_consensus.png}
         \caption{chessboard}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Blend_L5_consensus.png}
         \caption{Blend}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/clean_L5_consensus.png}
         \caption{Clean}
     \end{subfigure}
        \caption{Layer-5 consensus, $\sigma/\|\mu\|$}
        \label{fig:layer5-consensus}
\end{figure*}

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/BadNet_L5_mu.png}
         \caption{BadNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/WaNet_L5_mu.png}
         \caption{WaNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Chess_L5_mu.png}
         \caption{chessboard}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Blend_L5_mu.png}
         \caption{Blend}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/clean_L5_mu.png}
         \caption{Clean}
     \end{subfigure}
        \caption{Layer-5 L2 norm of $\mu$, $\|\mu\|$}
        \label{fig:layer5-norm}
\end{figure*}

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/BadNet_L13_consensus.png}
         \caption{BadNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/WaNet_L13_consensus.png}
         \caption{WaNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Chess_L13_consensus.png}
         \caption{chessboard}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Blend_L13_consensus.png}
         \caption{Blend}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/clean_L13_consensus.png}
         \caption{Clean}
     \end{subfigure}
        \caption{Layer-13 consensus, $\sigma/\|\mu\|$}
        \label{fig:layer13-consensus}
\end{figure*}

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/BadNet_L13_mu.png}
         \caption{BadNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/WaNet_L13_mu.png}
         \caption{WaNet}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Chess_L13_mu.png}
         \caption{chessboard}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/Blend_L13_mu.png}
         \caption{Blend}
     \end{subfigure}
     \begin{subfigure}[b]{0.18\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/clean_L13_mu.png}
         \caption{Clean}
     \end{subfigure}
        \caption{Layer-13 L2 norm of $\mu$, $\|\mu\|$}
        \label{fig:layer13-norm}
\end{figure*}


